Rise of Distributed Deep Learning Training in the Big Model Era: From a Software Engineering Perspective

Deep learning (DL) has become a key component of modern software. In the "big model" era, the rich features of DL-based software substantially rely on powerful DL models, e.g., BERT, GPT-3, and the recently emerging GPT-4, which are trained on the powerful cloud with large datasets. Hence, training effective DL models has become a vital stage in the whole software lifecycle. When training deep learning models, especially those big models, developers need to parallelize and distribute the computation and memory resources amongst multiple devices in the training process, which is known as distributed deep learning training, or distributed training for short. However, the unique challenges that developers encounter in distributed training process have not been studied in the software engineering community. Given the increasingly heavy dependence of current DL-based software on distributed training, this paper aims to fill in the knowledge gap and presents the first comprehensive study on developers' issues in distributed training. To this end, we analyze 1,131 real-world developers' issues about using these frameworks reported on Stack Overflow and GitHub. We construct a fine-grained taxonomy consisting of 30 categories regarding the fault symptoms and summarize common fix patterns for different symptoms. Based on the results, we suggest actionable implications on research avenues that can potentially facilitate the distributed training to develop DL-based software, such as focusing on the frequent and common fix patterns when designing testing or debugging tools, developing efficient testing and debugging techniques for communication configuration along with the synthesis of network configuration analysis, designing new multi-device checkpoint-and-replay techniques to help reproduction, and designing serverless APIs for cloud platforms.

==> sections/tool.tex <==
\section{\sysname: A Preliminary Tool}
\label{tool}
%\czp{Please move this section before the implication section. We first demonstrate the usefulness of our findings by implementing a preliminary tool, then discuss further implications.}
%\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/tool_example.pdf}
    \caption{Example code of \sysname.}
    \label{fig:tool_example}
\end{figure}
%\end{comment}
We demonstrate the practical usefulness of our findings with a preliminary proof-of-concept debugging tool, \emph{\sysname}, which helps detect and fix common faults and provides debugging suggestions for developers in distributed training.
For demonstration, we implement \sysname for PyTorch, one of the most popular frameworks for both industry- and research-oriented developers \cite{frameworks1, frameworks2, frameworks3, frameworks4}.

We implement five most common fix patterns (according to F.4 and F.5 in Table~\ref{tab:finding}) in \sysname. %These fix patterns fixes 47.72\% of the faults in our whole dataset. %and 29 of the 30 fault symptom categories in our taxonomy. 
%\xzl{Reads like 1 fault symptom leads to 52.27\% faults in our dataset? If so, this symptom should be very significant.....}
\begin{itemize}[leftmargin=*]
\item For \textit{fixing framework version/installation} and \textit{fixing dependency version/installation}, \sysname checks if the framework version meets the hardwares' requirement and if the dependencies' versions meet the framework's requirement.
\item For \textit{fixing communication configuration}, \sysname records the configurations in code as well as communication-related environmental variables (inspired by I.7), and then detects communication-related faults and fixes some of them based on the collected runtime information. 
\item For \textit{fixing distributed API usage}, \sysname checks the arguments passed to the distributed-specific APIs as well as the order in that related APIs are called. It fixes the wrongly set arguments and calls the missing APIs. 
\item For \textit{fixing device assignment}, \sysname checks the device assignment of every input data and model.
\end{itemize}

Apart from detecting and fixing the aforementioned faults, \\ \sysname also records logs and environmental information for pinpointing potential issues. According to the recorded logs and information, \sysname provides debugging suggestions to developers as a supplement of logs from the original framework, which further helps developers to resolve their encountered issues.
\begin{comment}
\begin{figure*}
	\centering
	\vspace{-0.1in}
	\subfloat[Example code of PyTorch distributed training.]{
		\begin{minipage}[b]{0.5\linewidth}
		\includegraphics[width=1\linewidth]{figures/pytorch_example.pdf}
		\end{minipage}
	}
	\subfloat[Example code of the preliminary tool.]{
		\begin{minipage}[b]{0.5\linewidth}
			\includegraphics[width=1\linewidth]{figures/tool_example.pdf}
		\end{minipage}
	}
	\vspace{-0.1in}
	\caption{Example of the usage of \sysname.}
	%\vspace{-0.1in}
	\label{fig:tool_example}
\end{figure*}
\end{comment}

\sysname provides out-of-box APIs for developers to debug their distributed training programs. The APIs are compatible with the APIs provided in PyTorch.
% , e.g., \textit{init\_process\_group()}, \textit{DistributedSampler()}, \textit{DataLoader()}, and \textit{DistributedDataParallel()}. 
Figure \ref{fig:tool_example} shows an example code snippet of \sysname. 
To use \sysname, developers need to (1) locate their code where uses the APIs that are specific to distributed training, and change them to the corresponding APIs provided by \sysname; 
(2) wrap the code to test in a function. Specifically, the APIs to be modified include communication setup APIs (line 3-5, which is essential for multi-device cooperation), data preparation APIs (line 6-8, which involve in data partition), and model preparation APIs (line 11-12, which involve in model partition and aggregation), etc.
%Specifically, developers need to modify: (1) communication setup API (line 3-5). The API is essential for the cooperation between devices. Here, we check the communication configuration, API usage, and device assignment of the worker; (2) data preparation APIs (line 6-8). These APIs involve in data shuffle and partition across workers. We mainly check the API usage according to a few patterns; (3) model preparation API (line 11-12). The wrapped DL model aggregates gradients in the training process. We check the arguments according to a few patterns and if the model and data are on the correct device. Besides, 
\sysname performs checks in each of these APIs according to the patterns we summarized.
More usage instructions of \sysname and implementation details can be found in our project repository~\cite{DTClinic}.

Although we only performed checks according to a few commonly encountered patterns, \sysname can detect issues or give debugging suggestions on 38\% of the collected faults using PyTorch. 
\sysname can successfully detect commonly-encountered faults including  communication errors~\cite{pytorch38300}, hang~\cite{pytorch28257}, and tensor mismatch~\cite{pytorch25267}. Some faults such as device error~\cite{pytorch46821} and communication error~\cite{pytorch31035} can be fixed by \sysname. 
Besides, \sysname provides program logs, which can help debug more potential issues.
%\xzl{How many reported bugs in  issues are covered in our case? How many bugs? A brief summary is appreciated.}

Note that currently \sysname is only implemented as a preliminary tool to demonstrate the usefulness of our findings. Because few reproducible and complete code samples can be collected from SO and GitHub, it prevents us from making a thorough test of \sysname. 
It is also worth mentioning that \sysname can be easily extended to other frameworks and can be extended to detect or fix more types of faults in distributed training. We leave the extension of \sysname for future work.

